What Do Speech Foundation Models Not Learn About Speech?

Understanding how speech foundation models capture non-verbal cues is crucial for improving their interpretability and adaptability across diverse tasks. In our work, we analyze several prominent models such as Whisper, Seamless, Wav2Vec, HuBERT, and Qwen2-Audio focusing on their learned representations in both paralinguistic and non-paralinguistic tasks from the Dynamic-SUPERB benchmark. Our study addresses three key questions: (1) What non-verbal cues (e.g., speaker intent, emotion, environmental context) are captured? (2) How are these cues represented across different layers of the models? and (3) To what extent can these representations be effectively adapted to downstream tasks? To answer these questions, we first evaluate the models in a zero-shot setting, followed by fine-tuning on layer-wise features extracted from these models. Our results provide insights into the models' capacity for generalization, the characteristics of their layer-wise representations, and the degree of transformation required for downstream task adaptation. Our findings suggest that some of these models perform well on various tasks in zero-shot settings, despite not being explicitly trained for those tasks. We also observe that zero-shot performance correlates with better-learned representations. The analysis of layer-wise features demonstrates that some models exhibit a convex relationship between the separability of the learned representations and model depth, with different layers capturing task-specific features.

==> plots/zero-shot-radar.tex <==
\begin{figure}[hbt]
    \centering
    \includegraphics[width=1.\linewidth]{assets/radar-chart.pdf}
    \caption{Zero-shot results.}
    \label{fig:zero-shot}
\end{figure}

==> tables/results-main.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{lllllllllll}
\toprule
Setting                                  & W-L-v3 & W-l-v2 & DW-v2 & DW-v3 & W-M & W-M-en & W-S & W-S-en & W-B & W-B-en \\ \midrule
Zero-Shot                                &        &        &       &       &     &        &     &        &     &        \\ \hdashline
\multicolumn{1}{c}{\multirow{6}{*}{KNN}} & en-0   &        &       &       &     &        &     &        &     &        \\
\multicolumn{1}{c}{}                     & en-l/2 &        &       &       &     &        &     &        &     &        \\
\multicolumn{1}{c}{}                     & en-l   &        &       &       &     &        &     &        &     &        \\
\multicolumn{1}{c}{}                     & de-0   &        &       &       &     &        &     &        &     &        \\
\multicolumn{1}{c}{}                     & de-l/2 &        &       &       &     &        &     &        &     &        \\
\multicolumn{1}{c}{}                     & de-l   &        &       &       &     &        &     &        &     &        \\ \hdashline
\multicolumn{1}{c}{\multirow{6}{*}{KNN}}                     & en-0   &        &       &       &     &        &     &        &     &        \\
                                         & en-l/2 &        &       &       &     &        &     &        &     &        \\
                                         & en-l   &        &       &       &     &        &     &        &     &        \\
                                         & de-0   &        &       &       &     &        &     &        &     &        \\
                                         & de-l/2 &        &       &       &     &        &     &        &     &        \\
                                         & de-l   &        &       &       &     &        &     &        &     &   \\ \bottomrule     
\end{tabular}
\caption{ \label{tab:results_main}
Results main.
}
\end{table*}



==> tables/task-results.tex <==
\begin{table*}[]
\begin{tabular}{lllllllllll}
\toprule
Task   & W-L-v3 & W-l-v2 & DW-v2 & DW-v3 & W-M & W-M-en & W-S & W-S-en & W-B & W-B-en \\ \midrule
Task1  & ZS/K/D &        &       &       &     &        &     &        &     &        \\
Task2  &        &        &       &       &     &        &     &        &     &        \\
Task3  &        &        &       &       &     &        &     &        &     &        \\
Task4  &        &        &       &       &     &        &     &        &     &        \\
Task5  &        &        &       &       &     &        &     &        &     &        \\
Task6  &        &        &       &       &     &        &     &        &     &        \\
Task7  &        &        &       &       &     &        &     &        &     &        \\
Task8  &        &        &       &       &     &        &     &        &     &        \\
Task9  &        &        &       &       &     &        &     &        &     &        \\
Task10 &        &        &       &       &     &        &     &        &     &    \\

\bottomrule
\end{tabular}
\caption{ \label{tab:task_results}
Task Results.
}
\end{table*}
